Making Sense of Constellations: Methodologies for Understanding Starlink's Scheduling Algorithms

Starlink constellations are currently the largest LEO WAN and have seen considerable interest from the research community. In this paper, we use high-frequency and high-fidelity measurements to uncover evidence of hierarchical traffic controllers in Starlink -- a global controller which allocates satellites to terminals and an on-satellite controller that schedules transmission of user flows. We then devise a novel approach for identifying how satellites are allocated to user terminals. Using data gathered with this approach, we measure the characteristics of the global controller and identify the factors that influence the allocation of satellites to terminals. Finally, we use this data to build a model which approximates Starlink's global scheduler. Our model is able to predict the characteristics of the satellite allocated to a terminal at a specific location and time with reasonably high accuracy and at a rate significantly higher than baseline.

==> Makefile <==
# Makefile for LaTeX files
# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile
# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.
# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo
# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 
# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 
# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $
LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"
DATE=$(shell date +%Y-%m-%d)
COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false
# These are OK
SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)
# These are not
#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))
define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef
define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef
define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef
define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef
define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef
define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef
all 	: $(TRG)
.PHONY	: all show clean ps pdf showps veryclean
clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)
veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~
# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 
include $(SRC:.tex=.d)
# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)
$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@
#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
#$(PDF) : %.pdf : %.tex
#	@$(run-pdflatex)
show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done
showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done
ps	: $(PSF) 
pdf	: $(PDF) 
# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)
######################################################################
# Define rules for EPS source files.
# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12
#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))

==> tex/experiments.tex <==
\section{Experiments}\label{sec:experiments}



\subsection{Understanding performance characteristics intrinsic to Starlink}
\label{sec:experiments:characteristics}

\textbf{Fine-grained observations}
\\
Starlink constellations make scheduling decisions, i.e what satellite serves which cell, every 15 seconds. This can theoretically result in different performance (latency + packet loss) during every 15 second slot. Previous studies have made observations which are too coarse-grained, either by binning data into slots > 15s or computing higher-level statistics over the entire data set (days or weeks), to draw out any regular changes in performance.
\\
\textbf{Figure out at what offsets these 15 seconds slots start}
Could we just go by visual observations? Not a bad idea given this offset can only start from 15 different points after the minute. 
\\
Maybe - 15 second sliding window to observe which window offsets give us the most stable performance within each slot. But what about slots with random rtts?

\textbf{Takeaway} 15 second slots start at 12, 27, 52 and 57 seconds after the minute 
\\
\textbf{Fine-grained measurements}
\\
In the previous experiment, we observed that studies that use coarse-grained observations to characterise starlink performance miss out on regular changes in starlink performance. Now, we want to analyse whether any patterns exist within each 15 second slot. Every 15 second slot, a different satellite connected to a different gateway could be potentially serving our dish. As different satellites are serving different amounts of customers + traffic, we expect different patterns within each 15 second slot. 
\\
To characterise different behaviours, we conduct fine-grained measurements (reasoning: because MAC scheduler schedules packets in bursts with limited space in radio frames, we wanted to observe how this scheduling works).
\begin{itemize} 
		\item Latency measurements using IRTT for different interval granularities (10,20,50,100,1000ms)
		\item IPerf for different throughputs
\end{itemize}

IPerf for different throughputs
We use scagnostics - which extracts features from the distribution of RTTs over time in a 2d space - to cluster these behaviours

Types of clusters we observe:
\begin{itemize} 
		\item Band formation
		\item Random
		\item Diagonal pattern
		\item Satellite failures - switch from an existing pattern to another within each 15 second slot
\end{itemize}

Digging deeper into why bands form?
Hypothesis: Bands should form when there is not enough space in the current burst/radio frame to fit all of a single user’s traffic

\subsection{Implications of performance characteristics on performance measurements}
\label{sec:experiments:implications}
What do coarse-grained observations miss about starlink performance?
Starlink connection’s performance can vary a lot from one slot to another (distribution of differences) 
\\
Compare the performance observed within each 15 second slot and compare it to the average statistics that would be reported by a more coarse-grained analysis. Example: Although the analysis shows that on average starlink performs better than cable internet, we show that within x 15 second slots, it's worse (or better).
\\
Compare distribution of differences between 15 second slots vs x second slots used by a more coarse-grained analysis. Fine-grained should show more drastic changes.
\\

\textbf{Implications on applications}
\begin{itemize} 
		\item VoIP
		\item Gaming
\end{itemize}
